DeepMerge: Learning to Merge Programs

In collaborative software development, program merging is the mechanism to integrate changes from multiple programmers. Merge algorithms in modern version control systems report a conflict when changes interfere textually. Merge conflicts require manual intervention and frequently stall modern continuous integration pipelines. Prior work found that, although costly, a large majority of resolutions involve re-arranging text without writing any new code. Inspired by this observation we propose the first data-driven approach to resolve merge conflicts with a machine learning model. We realize our approach in a tool DeepMerge that uses a novel combination of (i) an edit-aware embedding of merge inputs and (ii) a variation of pointer networks, to construct resolutions from input segments. We also propose an algorithm to localize manual resolutions in a resolved file and employ it to curate a ground-truth dataset comprising 8,719 non-trivial resolutions in JavaScript programs. Our evaluation shows that, on a held out test set, DeepMerge can predict correct resolutions for 37% of non-trivial merges, compared to only 4% by a state-of-the-art semistructured merge technique. Furthermore, on the subset of merges with upto 3 lines (comprising 24% of the total dataset), DeepMerge can predict correct resolutions with 78% accuracy.

==> background.tex <==
\section{Why a data-driven program merge?}

\subsection{Problem formulation: Intuition}
Loosely defined in terms of ``intent''

\subsection{Problem formulation in terms of runtime semantics}
Semantic conflict freedom. Too strict. 

\subsection{Existing solutions}

Discuss the existing solutions and their shortcomings. 

\subsubsection{Unstructured (text-based) merge}
No understanding of program syntax, let alone semantics. 
Show an example. 

\subsubsection{Structured merge}
Very language specific. 
Provide no solutions for statements

\subsubsection{Verified merge}

Very very language specific
Hard to work for dynamic languages
Will never work for non-Code, or semi-code (Docker), configuration files, 


==> code_highlight.tex <==


% this comes from https://tex.stackexchange.com/questions/15237/highlight-text-in-code-listing-while-also-keeping-syntax-highlighting/49309#49309

\makeatletter
\newenvironment{btHighlight}[1][]
{\begingroup\tikzset{bt@Highlight@par/.style={#1}}\begin{lrbox}{\@tempboxa}}
	{\end{lrbox}\bt@HL@box[bt@Highlight@par]{\@tempboxa}\endgroup}

\newcommand\btHL[1][]{%
	\begin{btHighlight}[#1]\bgroup\aftergroup\bt@HL@endenv%
	}
	\def\bt@HL@endenv{%
	\end{btHighlight}%   
	\egroup
}
\newcommand{\bt@HL@box}[2][]{%
	\tikz[#1]{%
		\pgfpathrectangle{\pgfpoint{1pt}{0pt}}{\pgfpoint{\wd #2}{\ht #2}}%
		\pgfusepath{use as bounding box}%
		\node[anchor=base west, fill=orange!25,outer sep=.5pt,inner xsep=0.5pt, inner ysep=-0.3pt, rounded corners=2pt, minimum height=\ht\strutbox-.1pt,#1]{\raisebox{.01pt}{\strut}\strut\usebox{#2}};
	}%
}
\makeatother

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}

\lstdefinelanguage{JavaScript}{
  keywords={typeof, new, true, false, catch, function, return, null, catch, switch, var, if, in, while, do, else, case, break},
  keywordstyle=\color{blue}\bfseries,
  ndkeywords={class, export, boolean, throw, implements, import, this},
  ndkeywordstyle=\color{darkgray}\bfseries,
  identifierstyle=\color{black},
  sensitive=false,
  comment=[l]{//},
  morecomment=[s]{/*}{*/},
  commentstyle=\color{purple}\ttfamily,
  stringstyle=\color{red}\ttfamily,
  morestring=[b]',
  morestring=[b]"
}

\lstdefinestyle{mystyle}{
% 	backgroundcolor=\color{backcolour}, 
	frame=single,  
	commentstyle=\color{codegreen},
	keywordstyle=\color{blue}\bfseries,
	numberstyle=\tiny\color{codegray},
	stringstyle=\color{codepurple},
	basicstyle=\linespread{0.75}\fontsize{5.8}{9.3}\ttfamily\bfseries,
	breakatwhitespace=false,         
	breaklines=false,                 
	captionpos=b,                    
	keepspaces=true,                 
% 	numbers=left,                    
	numbersep=3pt,                  
	showspaces=false,                
	showstringspaces=false,
	showtabs=false,                  
	tabsize=2,
% 	language=[Sharp]C,
	language=JavaScript,
	moredelim=**[is][{\btHL[fill=cyan!15]}]{/+a}{+/},
	moredelim=**[is][{\btHL[fill=cyan!60]}]{/+ae}{+/},
	moredelim=**[is][{\btHL[fill=green!60]}]{/+mybe}{+/},
	moredelim=**[is][{\btHL[fill=green!20]}]{/+b}{+/},
	moredelim=**[is][{\btHL[fill=gray!20]}]{/+o}{+/},
	moredelim=**[is][{\btHL[fill=red!40]}]{/+e}{+/},
}



==> frontmatter.tex <==
\acmJournal{PACMPL}
\acmVolume{1}
\acmNumber{POPL} 
\acmArticle{1}
\acmYear{2018}
\acmMonth{1}
\acmDOI{} % \acmDOI{10.1145/nnnnnnn.nnnnnnn}
\startPage{1}

\setcopyright{none}


==> impl.tex <==
\subsection{Training \deepMergeTool}
% In the prior sections, Section~\ref{sec:input} discussed how it solves
% \challenge{1}, how to represent edits for a sequence-to-sequence
% model, with \textit{Merge2Matrix}.  Likewise, Section~\ref{sec:output}
% discussed how it solves \challenge{2}, how to copy segments from the
% input to output.  This section describes how we use these constituents
% in a larger sequence model.  

% \deepMergeTool{} takes a merge tuple (($A, B, O$), $R_\bot$) and
% encodes ($A, B, O$) into a matrix with \textit{Merge2Matrix}.  It then
% uses a bidirectional GRU\cite{} to encode

The prior sections discussed the overall model architecture of
\deepMergeTool.  Assume the model parameters are contained in
$\theta$; training seeks to find the values of $\theta$ that maximize
the log-likelihood
$$\argmax_{\theta} \log p_{\theta}(R | A, B, O)$$
over all merge tuples (($A, B, O$), $R$) in its training
dataset.  We use standard cross-entropy loss with the Adam optimizer.
Training takes roughly 18 hours on a NVIDIA P100 GPU and we pick the
model with the lowest validation loss, which occurred after \TODO{Y}
epochs.  

%\subsection{Beam Search}
%Do we talk about this?


==> intro_old.tex <==
% !TeX root = ./main.tex
\newcommand{\baseProg}{\mathcal O}
\newcommand{\aProg}{\mathcal A}
\newcommand{\bProg}{\mathcal B}
\newcommand{\resProg}{\mathcal M}
\newcommand{\mergeProg}{\mathcal C}
\newcommand{\edit}[1]{\Delta_{#1}}
\newcommand{\aEdit}{\edit{\aProg}}
\newcommand{\bEdit}{\edit{\bProg}}
\newcommand{\resEdit}{\edit{\resProg}}

\newcommand{\diffThree}{{\tt diff3}}
\newcommand{\safeMergeTool}{{\sc SafeMerge}}

\newcommand{\var}[1]{{\tt #1}}
\newcommand{\challenge}[1]{{\bf CH{#1}}}

\section{Introduction}
\label{sec:introduction}

Program merging is an integral part of any software
development lifecycle that involves collaboration between
multiple developers. 
According to a large scale empirical study of Java projects on
GitHub~\cite{ghiotto-tse18}, almost 12\% of all commits
are related to a merge.  

A merge is a rare instance where developers use an algorithm to
rewrite programs.
Formally, a {\it three-way program merge} algorithm takes as
input two programs $\aProg$ and $\bProg$ obtained by modifying a
common {\it base} program $\baseProg$, and either:
\begin{enumerate}
\item provides a merged program $\resProg$ that preserves the ``intent''
of the changes made in $\aProg$ and $\bProg$ over $\baseProg$, or
\item declares a ``conflict'' if the two changes may interfere with each other. 
\end{enumerate}
A common manifestation of such a merge algorithm is in
the {\it git merge} command that is used to integrate changes across
two branches or forks in a version control system.

\begin{comment}
A central challenge in designing a merge algorithm is how to capture
the abstract notion of ``intent'' of a program change.
Existing approaches can accordingly be broadly classified into semantic or textual.
We use the two examples depicted in Figure \ref{fig:intro:example}
to illustrate how these two kinds of approaches attempt to capture intent
and what problems they entail.
\end{comment}

\begin{comment}
\begin{figure}
% git merge-file --diff3 -p 1_a.js 1_base.js 1_b.js
\footnotesize{
\begin{tabular}{@{}llllll@{}}
& \multicolumn{1}{c}{\underline{Base $\baseProg$}} &
  \multicolumn{1}{c}{\underline{Variant $\aProg$}} &
  \multicolumn{1}{c}{\underline{Variant $\bProg$}} &
  \multicolumn{2}{c@{}}{\underline{Merge Result $\resProg$}} \\
& \multicolumn{1}{c}{({\tt base.js})} &
  \multicolumn{1}{c}{({\tt a.js})} &
  \multicolumn{1}{c}{({\tt b.js})} &
  \multicolumn{1}{c}{{\it semantic}} &
  \multicolumn{1}{c@{}}{{\it textual} ({\tt diff3})} \\
\hline

                 & {\tt\ y = 42;}  & {\tt\ x = 1;}  & {\tt\ z = 43;} & {\tt\ \ x = 1;}  &                        \\
{\bf (1).}       &                 & {\tt\ y = 42;} & {\tt\ y = 42;} & {\tt\ \ z = 43;} & \ \ \ \ \ ``conflict'' \\
                 &                 &                 &                & {\tt\ \ y = 42;} & \\
\hline
                 & {\tt\ y = 42;} & {\tt\ x = 1;}   & {\tt\ y = 42;} &               &\ \ \ \ \ {\tt x = 1;}  \\
{\bf (2).}       & {\tt\ z = 43;} & {\tt\ y = 42;}  & {\tt\ x = 2;}  & \ \ ``conflict''  &\ \ \ \ \ {\tt y = 42;} \\
                 &                & {\tt\ z = 43;}  & {\tt\ z = 43;} &               &\ \ \ \ \ {\tt x = 2;}  \\
                 &                &                 &                &               &\ \ \ \ \ {\tt z = 43;} \\
\hline
\end{tabular}}
\vspace{-0.1in}
\caption{Two examples of three-way program merges with different merge results by
semantic and textual approaches. \label{fig:intro:example}}
\vspace{-0.3in}
\end{figure}
\end{comment}


\begin{figure}
% git merge-file --diff3 -p 1_a.js 1_base.js 1_b.js
\footnotesize{
\begin{tabular}{@{}llllll@{}}
& \multicolumn{1}{c}{{Base $\baseProg$}} &
  \multicolumn{1}{c}{{Variant $\aProg$}} &
  \multicolumn{1}{c}{{Variant $\bProg$}} &
  \multicolumn{1}{c}{{Spurious?}} \\
& \multicolumn{1}{c}{{\tt (base.js)}} & 
  \multicolumn{1}{c}{{\tt (a.js)}}  & 
  \multicolumn{1}{c}{{\tt (b.js)}} & \\
\hline
                 &                 &                 &                & \\
{\bf (1).}       & {\tt\ x = 0;} & {\tt\ x = 1;}   & {\tt\ x = 2;} &  {\tt No} \\ 
                 &                 &                 &                & \\
\hline
                 &                 &                 &                & \\
                 & {\tt\ y = 42;}  & {\tt\ x = 1;}  & {\tt\ z = 43;} &   {\tt Yes} \\
{\bf (2).}       &                 & {\tt\ y = 42;} & {\tt\ y = 42;} &  \\
                 &                 &                 &               &  \\
\hline
\end{tabular}}
%\vspace{-0.1in}
\caption{Two examples of merge conflicts. \label{fig:intro:example}}
%\vspace{-0.3in}
\end{figure}


% Merge conflicts are an issue
% Example (2)
% However, conflicts may be spurious
% Example (1)
% A large number are spurious: most resolutions take lines from A/B
The merge algorithm in widespread use in modern version control systems such as {\it git} is the \diffThree{} algorithm \cite{smith-98}.
The algorithm performs a three-way merge by treating documents as list-structured data. 
Intuitively, this algorithm {\it aligns} the two-way diffs of $\aProg$ (resp. $\bProg$)
over the common base~$\baseProg$ into a sequence of diff slots, and incorporates
the textual change from one of $\aProg$ or $\bProg$ at each slot unless both
programs change a common slot.
In the latter case, a (textual) merge conflict is produced that requires manual
resolution of the conflicting textual changes.

Merge conflicts are consistently ranked as one of the most difficult issues in collaborative software development~\cite{bachelli-et-al}.
Let us illustrate such conflicts with two simple code snippets in Figure~\ref{fig:intro:example}.
The Figure shows the base program $\baseProg$ along with the two variants $\aProg$ and $\bProg$ respectively. 
Example (1) shows a case where \diffThree{} detects a true conflict as the two branches change the value of a common variable {\tt x} differently.
This is useful issue to flag to a developer, as the only way to resolve this conflict will require the authors to agree between one of the two changes. 
On the other hand, example (2) shows a case where \diffThree{} declares a conflict because two independent and non-interfering changes (updates to {\tt x} and {\tt z}) are overlapping at the textual level. 
There are several ways to resolve the conflict by concatenating the changes from $\aProg$ and $\bProg$ in either order.
We call such merge conflicts that solely arise due to a specific representation of the input (in this case, line-based) as {\it spurious merge conflicts}. 
Such spurious merge conflicts severely slow down developer productivity, results in broken builds and often stall the continuous integration (CI) pipelines for several days~\cite{zimmermann-cite}. 

% prior works have been semantic, but requires logic
% structured and semi-structured merge deal with structure, cannot deal with semantics,
The issue of such spurious merge conflicts has inspired research to incorporate a programs structuce and semantics into account to perform merges.
Structured merge approaches~\cite{Apel11, lessenich2015} and variants treat merge inputs as abstract syntax trees (ASTs), and use tree-based matching and merge algorithms.
However, such approaches still yield a conflict on examples such as (2) above, as they do not model program semantics and cannot safely reorder statements inside a method that have side effects.
On the other hand, semantics based approaches can be used to alleviate this problem by formulating a notion of {\it semantic-conflict freedom}~\cite{Yang1992,Sousa18}.
However, no tools exist for a real-world programming language that can synthesize a merge; Sousa et al.~\cite{Sousa18} build a tool that can only verify if a merge is conflicting.
In this paper, we only concern with spurious merge conflicts produced by tools present in {\it git}; do not address the issue of silent merges performed by \diffThree{} that may lead to structural or semantic conflicts~\cite{Sousa18}.

% Motivated by this observation, we ask the following question:
% given a merge conflict, can we predict it is a true conflict or a spurious conflict
% moreover, for a spurious conflict, we would like the resolution
% we don't address the issue of silent merges that may induce build, test or regressions.


% in this work, we pose it as a machine learning problem: data-driven merge

\begin{comment}
\paragraph{Existing Merge Algorithms.}
According to an intuitive formal notion in the literature \cite{Yang1992,Sousa18},
the ``intent'' of a change is defined as the set of program executions
whose observable output values are altered by the change.
Then, two programs $\aProg$ and $\bProg$ make conflicting changes
if and only if they both alter the behavior of an output variable in a common execution.
Based on this definition, the changes in Example (1) are not conflicting,
yielding the merge result $\resProg$ in the {\it semantic} column.
On the other hand, the changes in Example (2) are conflicting, since
$\aProg$ and $\bProg$ both modify the value of variable {\tt x} on a trace differently.

Such semantic notions of intent have given rise to merge frameworks that aim
to ensure correct merges by leveraging program analysis based techniques \cite{Yang1992,Sousa18}.
However, these solutions are limited in terms of scalability and expressiveness.
For instance, dynamic features such as reflection (in Java) and \texttt{eval} (in JavaScript)
make static verification infeasible.
Furthermore, these notions of intent are imperfect; for instance, they do not take
into account attributes of the syntax that may be valuable for maintenance,
including coding conventions regarding variable and method naming.

Due to these drawbacks of semantic approaches, the merge algorithms in widespread
use treat programs as list-structured textual data, and are agnostic of the syntax
or semantics of any programming language.
The most prevalent such algorithm, underlying {\it git} and other version control
systems, is the \diffThree{} algorithm \cite{smith-98}.
Intuitively, this algorithm {\it aligns} the two-way diffs of $\aProg$ (resp. $\bProg$)
over the common base~$\baseProg$ into a sequence of diff slots, and incorporates
the textual change from one of $\aProg$ or $\bProg$ at each slot unless both
programs change a common slot.
In the latter case, a (textual) merge conflict is produced that requires manual
resolution of the conflicting textual changes.

The difficulty of formalizing the notion of ``intent'' of a program change for
text introduces a different set of problems for textual approaches compared to
those for semantic approaches:
``spurious'' merge conflicts and silent ``bad'' merges.
For instance, running the command:
{\small
\begin{verbatim}
      git merge-file --diff3 -p a.js base.js b.js
\end{verbatim}
}
\noindent on Example (1) above produces a spurious merge conflict shown in
Figure \ref{fig:intro:conflict}(a).
Such merge conflicts, comprising 12.4\% of all merges~\cite{ghiotto-tse18},
impact developer productivity and stall continuous integration and delivery
(CI/CD) pipelines for hours to days until they are manually resolved.
On the other hand, for Example (2), \diffThree{} silently produces
the bad merge shown in the {\it textual} column of Figure \ref{fig:intro:example}.
Such merges result in costly broken builds~\cite{brun-fse11}
or introduce bugs silently. 
\end{comment}

\begin{figure}
\begin{subfigure}[t!]{85pt}
{\footnotesize
\begin{tabular}{l}
\text{\text{\{ unchanged lines (prefix) \}}} \\
{\tt <{}<{}<{}<{}<{}<{}<} \\
\text{\textsf{\{ lines edited by $\mathcal{A}$ \}}} \\
{\tt |||||||} \\
\text{\textsf{\{ affected lines of base $\mathcal{O}$ \}}} \\
{\tt =======} \\
\text{\textsf{\{ lines edited by $\mathcal{B}$ \}}} \\
{\tt >{}>{}>{}>{}>{}>{}>} \\
\text{\textsf{\{ unchanged lines (suffix)} \}}
\end{tabular}
}
\caption{Format of a conflict.}
\end{subfigure}
\begin{subfigure}[t!]{80pt}
{\footnotesize
\begin{verbatim}
    <<<<<<< a.js
    x = 1;
    ||||||| base.js
    =======
    z = 43;
    >>>>>>> b.js
    y = 42;
\end{verbatim}}
\vspace{0.3in}
\caption{Conflict (I).}
\end{subfigure}
\begin{subfigure}[t!]{70pt}
{\footnotesize
\begin{verbatim}
  <<<<<<< a.js
  x = 1;
  w = 42;
  ||||||| base.js
  y = 42;
  =======
  z = 43;
  w = 42;
  >>>>>>> b.js
\end{verbatim}}
\vspace{0.03in}
\caption{Conflict (II).}
\end{subfigure}
\vspace{-0.1in}
\caption{Conflict format and two instances reported by \diffThree{}:
(I) in Example (1) of Figure \ref{fig:intro:example}, and
(II) in its variation where {\tt y} in {\tt base.js} is renamed
{\tt w} in both {\tt a.js} and {\tt b.js}. \label{fig:intro:conflict}}
\vspace{-0.1in}
\end{figure}

\begin{comment}
A third category of approaches perform a structured merge by operating on
the program's abstract syntax trees (ASTs)~\cite{Apel11, lessenich2015}.
They exploit the fact that certain AST nodes can be reordered in a tree for a given language.
This eliminates a class of spurious merge conflicts such as that in Example (1) above.
However, most statements within a method cannot be reordered.
Lastly, semi-structured merge approaches combine structured merge with textual
merge within method bodies, but inherit most of the latter's
limitations~\cite{semi-structured-merge-cite}.
Besides, structured merge techniques employ sub-tree matching algorithms that
scale poorly with the size of programs. 
\end{comment}

\shuvendu{Rewrite introduction by staying away from semantic approaches, and silent merges, as this paper does not quite address those.}

\paragraph{Our Approach: Data-Driven Merge.}
% "intent" with data driven merge in this paper
The ostensibly intrac-table challenge of capturing the ``intent'' of program
changes leads us to seek a merge algorithm that is guided by real-world merge
and merge-conflict data.
%In other words, we investigate the following research question:
%\begin{quote}
%{\it Is it possible to design a data-driven three-way merge algorithm?}
%\end{quote}
Such a data-driven merge algorithm has the ability to achieve a
sweet-spot between a strict semantics based approach and a textual
approach, by learning from both successful merges as well as how
developers resolve conflicting merges.
\begin{comment}
\begin{enumerate}[leftmargin=*]
\item It can learn patterns that repeat in a given language
(e.g. {\it printf} statements can be reordered in most cases).
\item It can possibly be easily extended to multiple programming
languages, given recent advances in deep models for code such as
{\it code2vec}, {\it GPT-C}, and {\it CodeBERT}.
\item It has a better hope (compared to \diffThree{}) of producing
merge results that are well-formed and devoid of syntax and semantic errors.
\item It has the best chance to adapt to a project's unique
resolution patterns, which has been postulated as a useful quality
of a merge algorithm~\cite{ghiotto-tse18}.
\end{enumerate}
\end{comment}

We thereby formulate the ``data-driven three-way program merge''
problem as a machine learning problem, specifically a sequence-to-sequence
task akin to machine translation.
In our setting, the text of programs $\aProg$, $\bProg$, and $\baseProg$
corresponds to the input sequence, and the text of the resolved program
$\resProg$ corresponds to the output sequence.

We set out by identifying the challenges that a sequence-to-sequence model
must address to effectively learn a merge algorithm for a given language.
These challenges concern representing the merge inputs, constraining the 
output vocabulary, and obtaining unambiguous ground truth to train the model.
We then propose a data-driven merge tool \deepMergeTool{} that addresses
these challenges.

To address the challenge of input representation, \deepMergeTool{} employs an embedding 
of the merge inputs in a manner that is aware 
of $\aProg$'s and $\bProg$'s edits over the common base $\baseProg$.
We presume these edits are provided in the format of {\tt diff3} which is
depicted in Figure \ref{fig:intro:conflict}(a) in the portion between
markers ``{\footnotesize \verb+<<<<<<<+}'' and ``{\footnotesize \verb+>>>>>>>+}''.
Recall conflict (I) shown in Figure \ref{fig:intro:conflict}(b) which was
reported by {\it git merge} for Example (1).
This is a relatively simple conflict:
the portion between markers ``{\footnotesize \verb+|||||||+}'' and
``{\footnotesize \verb+=======+}'' is empty since no lines of base $\baseProg$
are affected.
Further, $\aProg$ and $\bProg$ only add a line each.
%{\small \verb+x = 1;+} and {\small \verb+z = 43;+} respectively.

On the other hand, consider a variant of Example (1) in which both $\aProg$ and $\bProg$
rename variable {\tt y} to {\tt w}.
The resulting conflict (II) is depicted in Figure \ref{fig:intro:conflict}(c).
Deriving the resolved program involves picking the line {\tt x = 1} in $\aProg$,
the line {\tt z = 43} in $\bProg$, and the line {\tt w = 42} in either, but not
the affected line {\tt y = 42} in $\baseProg$.
This example highlights that the merge inputs must be encoded in a manner that
is aware of the edits by $\aProg$ and $\bProg$ over base $\baseProg$.

Recent work has shown how to learn embeddings of
two-way program diffs \cite{yin2018learning}.
%Extending the idea to three-way program diffs is challenging.
Using their encoding, the edits of $\aProg$ and $\bProg$ over $\baseProg$
can be represented as the ``edit sequences'' (1) and (2) below, respectively:
\[
\begin{array}{@{}r@{\ \ \ }c@{\ \ \ }c@{\ \ \ }c@{\ \ \ }c@{\ \ \ }c@{\ \ \ }c@{\ \ \ }c@{\ \ \ }c@{\ \ \ }c@{\ \ \ }l@{}}
\mbox{$\aProg$:}                            & x & = &    1 & ; & \textbackslash n & w & = & 42 & ; & \\
\mbox{diff of $\aProg$ over $\baseProg$:}   & + & + &    + & + & | & \leftrightarrow & = & = & = & \ \ \,(1) \\
\mbox{$\baseProg$:}                         &   &   &      &   &   & y & = & 42 & ; & \\
\mbox{\,diff of $\bProg$ over $\baseProg$:} & + & + &   +  & + & | & \leftrightarrow & = & = & = & \ \ (2) \\
\mbox{$\bProg$:}                            & z & = & 43\! & ; & \textbackslash n & w & = & 42\! & ; & 
\end{array}
\]
where ``+'' denotes an addition, ``='' denotes a match,
``$\leftrightarrow$'' denotes a replacement, and ``$|$'' marks newlines.
Our key insight is to combine the embeddings of the two edit sequences
into a single sequence in a manner that is compact, so as to accommodate
large program changes, yet preserves edit-awareness.
Crucially, it suffices to only capture information about the {\it kinds}
of edits as opposed to individual tokens, greatly improving model efficacy.

To address the challenge of output vocabulary, we limit the space of 
resolved programs to sequences of line-based (i.e. newline-delimited)
segments occurring in the merge inputs.
This enables \deepMergeTool{} to leverage a pointer network \cite{NIPS2015_29921001} to
construct the resolved program by copying input segments.
The induced search space is nevertheless large and suffices to capture
the vast majority of manual resolutions of merge conflicts in practice.
For instance, reconsider conflict (II) in Figure \ref{fig:intro:conflict}(c).
The resolved program can be any sequence of elements in the set
$\{ ``{\tt x = 1;}", ``{\tt z = 43;}", ``{\tt w = 42;}" \}$.
It thereby admits the correct resolution which involves using each of these elements once.
Even presuming no repetition---which is allowed in our model---there are
16 possibilities for this simple instance.
Although the resolution in this case is relatively easy,
resolutions in practice involve interleaving, discarding, or even
duplicating input segments.

Finally, training a supervised model like \deepMergeTool{} requires
ground truth in the form of merge resolutions.
However, raw merge data of resolutions in a code corpus 
poses a host of challenges, as users may introduce extraneous code
changes, and even automated approaches may silently introduce
errors such as in the case of Example (2) in Figure~\ref{fig:intro:example}.
In any case, one of the goals of tools like \deepMergeTool{} is to improve in accuracy
upon prevalent automated approaches by leveraging latent semantic
information from manual resolutions.
We thereby introduce an algorithm for unambiguously
extracting regions from manual resolutions.

% solutions 
%\subsubsection*{\deepMergeTool{}: A data-driven merge tool}
%In this paper, describe \deepMergeTool{}, the first data-driven merge tool based on deep neural networks that addresses these challenges.
% above using a combination of novel embedding of the input, a variation of {\it pointer networks} to copy tokens from input, and pruning the output sequences by limiting the number of {\it context switches} between $\aProg$ and $\bProg$ in constructing the merge. 

In this paper, we apply \deepMergeTool{} to merge JavaScript programs.
Besides its popularity, JavaScript is notorious for its rich dynamic features,
and lacks tooling support.
We have created a high-quality dataset of 11,241 merge tuples that require non-trivial resolutions from 18,515 repositories in GitHub.
\deepMergeTool{} resolves $\textbf{34.2}$\%  of textual merge-conflicts on this dataset.
%Moreover, for merges limited to 3 (resp. 6) lines in the input constituting ~24\% (resp. 67\%) of our overall dataset, \deepMergeTool{} resolves $\textbf{76.0}$\% (resp. $\textbf{67.5}$\%) of conflicts.
Moreover, for merges limited to 3 lines in the input constituting ~24\% of our overall dataset, \deepMergeTool{} resolves $\textbf{76.0}$\%  of conflicts.
%     manual resolutions (~\S~\ref{sec:eval}).
%\deepMergeTool{} can also predict \textbf{69.8}\% (resp. \textbf{63.38}\%) of merges (resp. within size 3 - samples within size 3 consists of ) that cannot be resolved without requiring additional tokens. 

% contributions
\paragraph{Contributions.}
We summarize the contributions of our work:
\begin{enumerate}[leftmargin=*]
\item We define the data-driven merge problem and identify a set of
challenges for encoding it as a sequence-to-sequence supervised learning problem (\S~\ref{sec:formulation}).
\item We present a data-driven merge tool \deepMergeTool{} that uses
  edit-aware embedding to represent merge inputs and
  a variation of pointer networks to construct the resolved program (\S~\ref{sec:deepmerge}).
\item We derive a high-quality merge dataset for supervised learning by
  proposing an algorithm for unambiguously extracting resolution regions (\S~\ref{sec:dataset}).
\item We perform an extensive evaluation of \deepMergeTool{} on JavaScript programs
  and demonstrate that it can correctly resolve $\textbf{34.2}$\%
  (resp. $\textbf{76.0}$\%) of merge conflicts (resp. within size 3) that require
  non-trivial manual resolutions (\S~\ref{sec:eval}).

%\item We perform an extensive evaluation on 1,086 number of merge conflicts in \TODO{YY} JavaScript projects, and resolve $\textbf{21.6}$\% (resp. 63.4\%) of textual merge-conflicts (resp. within size 3 lines) that require non-trivial manual resolutions (~\S~\ref{sec:eval}).
\end{enumerate}

%\textbf{motivation}

%State of software development today: large teams simultaneously editing the same code base. 
%Merging code changes is burdensome and error prone.
%Cite various bugs introduced during this process. (this process being the manual resolution)

%===========
%\textbf{Things we want in a solution}

%\begin{enumerate}
%\item{accurate: high accuracy}
%\item{efficient: real-time / IDE}
%\item{general: support rich language features}
%\item{flexible: no need for spec (e.g. test cases)}
%\end{enumerate}

%=======
%\textbf{How its different than existing solutions}

%Existing works which attempt to automate the merging of uncoordinated changes can be classified into three categories:
%\begin{enumerate}
%\item{purely syntactic: gitmerge and diffThree}
%\item{AST-aware: lots of works.  But slow, don't always output a solution, and language-specific.}
%\item{program-semantics aware: testing/verification (Isil/Shuvendu's work and MergeResolver), but require specifications, etc.}
%\end{enumerate}
%=======


%Existing solutions ???
%These tools face notable challenges. We present several? examples to illustrate their limitations. Structured merge techniques (citaition) attempt to preserve semantics. In some languages we can reason about semantics to a certain extent. However, in general, these tools cannot reason about reordering statements as they may have side effects. Structured merge techniques fail in these cases and default to a manual merge. In dynamic languages such as Python and Javascript, the task of an AST aware merge is even more difficult. Moreover, this example provides an interesting challenge as the resolution contains contents from A and B interleaved. (rather than taking complete chunks)

%Existing methods are slow!

%\noindent\subsection*{Contributions}
%In summary, we make the following contributions:
%\begin{enumerate}
%\item We formulate merge conflict resolution as a deep learning sequence2sequence problem
%\item We provide a framework for automatically resolving merge conflicts through:
%	\begin{enumerate}
%	\item Novel encodings of the input for leveraging deep learning 
%	\item A variation on pointer networks that drastically shrinks the size of the output vocabulary
%	\item An extension to the beam search algorithm to limit the number of context switches between chunks
%	\end{enumerate}
%\item We present an algorithm for extraction of resolution regions and assigning labels to a resolution.
%\item We perform extensive evaluation on \shuvendu{XXX} number of merge conflicts over \shuvendu{YYY} JavaScript and Java projects, and illustrate that our technique significantly outperforms simple baselines.
%\item We provide a large multi-lingual dataset of XXXX merge conflicts and their resolutions
%\end{enumerate}





==> motivating-examples.tex <==
\section{Motivating Examples}
%
%challenges:
%- large search space 
%- most solutions are syntactically
%  valid and sometimes even semantically
%- distribution


We present several examples to illustrate the complexity of true resolutions in addidtion to the limitations of current three way merge tools.
\begin{enumerate}
\item The objective of a three way merge algorithm is to provide a merged program $\resProg$ that captures the edits from $\aProg$ and $\bProg$. 


 $\aProg$, depicted in Figure \ref{fig:med}, edits the $\baseProg$ by inserting two arguments to the \texttt{Array.prototype.slice.call} call while $\bProg$ leaves the call unchaged. Similarily, $\bProg$ inserts an argument to the \texttt{this.props.onDrop} function call while $\aProg$ leaves the call unchanged. The developer constructs $\resProg$ by taking the first line from $\aProg$ and the second line from $\bProg$. That is, the developer chooses the lines that differ from $\baseProg$.

\item Figure \ref{fig:hard} depicts a more difficult example. In this sample, $\aProg$ inserts two lines: \texttt{gulp.task('html', htmlTask)} and \texttt{module.exports = htmlTask} to register the \texttt{htmlTask} function and export it. $\bProg$ modifies the first line in $\baseProg$ to call the method \texttt{stream} on the \texttt{browserSync} method. The developer creates $\resProg$ in Figure ?  by arranging the changes such that $\bProg$'s changes are inserted prior to $\aProg$'s. The changes are ordered such that the \texttt{htmlTask} method is completed prior to registering and exporting it. Existing AST aware methods would declare a conflict on this example as they do not handle conflicts within a function.

%\item hard 2
\item Lastly, we provide an example of a sample that cannot be merged. Figure \ref{fig:oov} illustrates a merge that requires additional tokens not present in $\aProg$ or $\bProg$ in order to resolve. In this example, $\aProg$ modifiedd the number of passing test cases by 4, from \texttt{71315} to \texttt{71319}. $\bProg$ modified the number of passing test cases by increasing \texttt{71315} by 2 to \texttt{71317}. In combination, $\aProg$ and $\bProg$ added a total of 6. The true resulting merge modifies \texttt{71315} to the new token \texttt{71321} representing the 6 additional tokens added.

\begin{figure*}[htbp!]
	%\vspace{-0.07in}
	\begin{subfigure}{0.49\textwidth}
		\lstset{style=mystyle}
		\lstinputlisting[linewidth=7.96cm]{./examples/medium_merged.js}
		%\vspace{-0.1in}
		\caption{Conflicting merge}
		\label{fig:conflict}
	\end{subfigure}\hfill
	\begin{subfigure}{0.5\textwidth}
		\lstset{style=mystyle}
		\lstinputlisting[linewidth=7.96cm]{./examples/medium_resolved.js}
		%\vspace{-0.1in}
		\caption{Merge resolution}
		\label{fig:res}
	\end{subfigure}\hfill

	\caption{Example remove $\baseProg$ sample}
	\label{fig:med}
	%\vspace{-0.07in}
\end{figure*}

\begin{figure*}[htbp!]
	%\vspace{-0.07in}
	\begin{subfigure}{0.5\textwidth}
		\lstset{style=mystyle}
		\lstinputlisting[linewidth=7.96cm]{./examples/hard_large_merged.js}
		%\vspace{-0.1in}
		\caption{Conflicting merge}
		\label{fig:a}
	\end{subfigure}\hfill
	\begin{subfigure}{0.5\textwidth}
		\lstset{style=mystyle}
		\lstinputlisting[linewidth=7.96cm]{./examples/hard_large_resolved.js}
		%\vspace{-0.1in}
		\caption{Merge resolution}
		\label{fig:a}
	\end{subfigure}\hfill

	\caption{Example hard}
	\label{fig:hard}
	%\vspace{-0.07in}
\end{figure*}


%
%\begin{figure*}[htbp!]
%	\vspace{-0.07in}
%	\begin{subfigure}{0.5\textwidth}
%		\lstset{style=mystyle}
%		\lstinputlisting[linewidth=8.51cm]{./examples/hard2_merged.js}
%		\vspace{-0.1in}
%		\caption{Conflicting merge}
%		\label{fig:a}
%	\end{subfigure}\hfill
%	\begin{subfigure}{0.5\textwidth}
%		\lstset{style=mystyle}
%\lstinputlisting[linewidth=8.51cm]{./examples/hard2_resolved.js}
%		\vspace{-0.1in}
%		\caption{Merge resolution}
%		\label{fig:a}
%	\end{subfigure}\hfill
%
%\caption{Example hard 2}
%	\label{fig:hard2}
%	\vspace{-0.07in}
%\end{figure*}

\begin{figure*}[htbp!]
	%\vspace{-0.07in}
	\begin{subfigure}{0.5\textwidth}
		\lstset{style=mystyle}
		\lstinputlisting[linewidth=6.96cm]{./examples/oov_merged.js}
		%\vspace{-0.1in}
		\caption{Conflicting merge}
		\label{fig:a}
	\end{subfigure}\hfill
	\begin{subfigure}{0.5\textwidth}
		\lstset{style=mystyle}
		\lstinputlisting[linewidth=6.96cm]{./examples/oov_resolved.js}
		%\vspace{-0.1in}
		\caption{Merge resolution}
		\label{fig:a}
	\end{subfigure}\hfill

	\caption{Example oov}
	\label{fig:oov}
	%\vspace{-0.07in}
\end{figure*}

\end{enumerate}


==> result.tex <==
\section{Results}
\label{sec:eval}

\subsection{Prediction Results}

\begin{table}[t]
\resizebox{.5\textwidth}{!}{%
\begin{tabular}{c||c|c|c|c}
\toprule
 Architecture & Accuracy & Precision & Recall & F1 Score \\
\toprule
 %\cmidrule(l){1-5}
 Strategy A &  &  &  &  \\
 Strategy B & & & &  \\
 Strategy Base &  &  &  &   \\
 Strategy AB &  &  &  &  \\
 Strategy BA &  &  &  &  \\
 Random Strategy &  &  &  &  \\
 Weighted Random Strategy &  &  &  &  \\
 \hline
 \bottomrule
\end{tabular}
}
\vspace{1mm}
\caption{Naive Results \label{tab:full_result}}
\vspace{1mm}
\end{table}
\subsection{Synthesis Results}

\subsection{Discussion}


==> threats.tex <==
% !TeX root = ./main.tex
\subsection{Threats to Validity}

As with any empirical investigation, our choice of dataset may be impacted by threats to validity~\cite{mitchell2012research}.
We outline the key threats to validity and our mitigation strategies in this section.
% 
%\noindent\textbf{External Validity} is concerned with the generalizability of our results.
%To achieve generalizability, the sample data sets we train on and evaluate on must be representative of the population of merge conflict resolutions.
To ensure that our dataset consists of representative merges, we sampled merge conflict resolutions from over \TODO{1126} software repositories on GitHub.
Gathering data from GitHub indiscriminately can lead to both noise and bias.  
We address this by following the advice of Kalliamvakou~\emph{et al.}~\cite{kalliamvakou2014promises} and select projects that have recent activity, received a large number of stars (positive sentiment), and include a non-trivial number of contributors.
Finally, there may be more than one correct merge resolution, such that using the recorded resolution as the oracle is incomplete.

%In this context, the results of \deepMergeTool{} may actually be better than reported, as it may be producing resolutions that do not match the oracle, but are nonetheless correct.

%\noindent\textbf{Internal Validity} refers to the factors that may affect the reliability of the results of the experiments.
%For both training and evaluation of \deepMergeTool{}, we require an oracle for each merge conflict resolution.
%Fortunately, we have a wealth of historical merge conflicts and resolutions that occurred in practice and thus we are able to treat the actual recorded resolutions as the oracle.
%We note that two potential issues with this approach.
%First, developers may not always resolve a merge correctly.
%We manually investigated a sample of commits and did not see evidence of modifying the merges in subsequent commits.
%Second, there may be more than one correct merge resolution, such that using the recorded resolution as the oracle is incomplete.
%In this context, the results of \deepMergeTool{} may actually be better than reported, as it may be producing resolutions that do not match the oracle, but are nonetheless correct.

%In terms of implementation, we rely on existing, well vetted tooling in both our data collection and model implementation.
%For example, we identify differences and conflicts using the well known \texttt{diff3} tool and our models are all built using the PyTorch framework.
%While we cannot unequivally state that our implementation is free of errors, we are confident in it because we employ Q/A practices such as code review in our 
%development and we have manually investigated the results heavily.


